Modeling Multiple Normal Action Representations for Error Detection in Procedural Tasks

Error detection in procedural activities is essential for consistent and correct outcomes in AR-assisted and robotic systems. Existing methods often focus on temporal ordering errors or rely on static prototypes to represent normal actions. However, these approaches typically overlook the common scenario where multiple, distinct actions are valid following a given sequence of executed actions. This leads to two issues: (1) the model cannot effectively detect errors using static prototypes when the inference environment or action execution distribution differs from training; and (2) the model may also use the wrong prototypes to detect errors if the ongoing action label is not the same as the predicted one. To address this problem, we propose an Adaptive Multiple Normal Action Representation (AMNAR) framework. AMNAR predicts all valid next actions and reconstructs their corresponding normal action representations, which are compared against the ongoing action to detect errors. Extensive experiments demonstrate that AMNAR achieves state-of-the-art performance, highlighting the effectiveness of AMNAR and the importance of modeling multiple valid next actions in error detection. The code is available at https://github.com/iSEE-Laboratory/AMNAR.

==> draft.tex <==
\toedit{Error detection in procedural activities is essential for consistent outcomes in AR-assisted and robotic systems. Existing methods fail to adaptively model multiple normal action representations for each task step, limiting their ability to capture the full range of normal variations, especially when multiple valid next actions are possible. To address this limitation, we propose an Adaptive Multiple Normal Action Representation (AMNAR) framework. AMNAR predicts all valid next actions and reconstructs their corresponding normal action representations, which are compared against the ongoing action to detect errors. Extensive experiments demonstrate that our approach achieves state-of-the-art performance, highlighting the effectiveness of AMNAR and the importance of modeling multiple valid next actions in error detection.}





\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/sec1/Valid Action and Predict_cropped.pdf} 
    \caption{A figure showing potential actions and error detection pipeline of our method.}
    \label{fig:valid_action_and_predict}
\end{figure}

\subsection{Handling Multiple Valid Next Actions}

Our analysis indicates that the ``coffee'' task has the highest occurrence of multiple valid next actions. As shown in \cref{tab:error_detection_egoper}, AMNAR achieves an 18.2\% improvement in EDA and a 9.5\% increase in AUC for this task, compared to average improvements of 7.4\% and 6.5\% respectively. This suggests that AMNAR is particularly effective at detecting errors in tasks with multiple valid next actions.

Furthermore, we conducted an experiment focusing on non-deterministic actions---those preceded by steps with multiple valid next options---to validate our method's effectiveness in such scenarios. Using frame-wise error detection accuracy, as shown in \cref{tab:acc_non_deterministic_actions}, AMNAR achieves the highest overall accuracy (73.7\%), outperforming other variants and the EgoPED framework significantly. For individual tasks, AMNAR performs well, especially in ``Oatmeal'' and ``Coffee,'' with accuracies of 75.5\% and 76.7\%. These results demonstrate that our model is more adept at handling complex tasks with non-deterministic action sequences, highlighting the advantage of modeling multiple valid next actions.

As shown in \cref{fig:visualization}, we visualize a sample from the coffee task where AMNAR mitigates errors from ASM misclassification. Here, the ground truth action is ``Grind coffee for 20 seconds,'' but ASM incorrectly predicts ``Discard paper filter and coffee grounds.'' The EgoPER framework misclassifies it as erroneous due to incorrect prototype selection. In contrast, AMNAR selects the closest normal action representation, correctly identifying the action as normal, demonstrating robustness in scenarios with label ambiguity or multiple valid action paths.

\begin{table}[t]
\centering
\caption{Detection accuracy of non-deterministic actions in EgoPER dataset}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c c c c}
\toprule
Method & Quesadilla & Oatmeal & Pinwheel & Coffee & Tea & All \\
\midrule
EgoPED\cite{lee2024error} & \textbf{74.0} & 65.5 & 56.5 & 65.3 & 64.8 & 65.2 \\
AMNAR (w/o NARPM) & 60.2 & 61.4 & 61.3 & 72.5 & 63.4 & 63.8 \\
AMNAR (Random) & 57.9 & 63.8 & 61.7 & 71.5 & 57.6 & 62.5 \\
AMNAR & 73.8 & \textbf{75.5} & \textbf{66.8} & \textbf{76.7} & \textbf{75.6} & \textbf{73.7} \\
\bottomrule
\end{tabular}
}
\label{tab:acc_non_deterministic_actions}
\end{table}

